Most Probable Densest Subgraphs

Computing the densest subgraph is a primitive graph operation with critical applications in detecting communities, events, and anomalies in biological, social, Web, and financial networks. In this paper, we study the novel problem of Most Probable Densest Subgraph (MPDS) discovery in uncertain graphs: Find the node set that is the most likely to induce a densest subgraph in an uncertain graph. We further extend our problem by considering various notions of density, e.g., clique and pattern densities, studying the top-k MPDSs, and finding the node set with the largest containment probability within densest subgraphs. We show that it is #P-hard to compute the probability of a node set inducing a densest subgraph. We then devise sampling-based efficient algorithms, with end-to-end accuracy guarantees, to compute the MPDS. Our thorough experimental results and real-world case studies on brain and social networks validate the effectiveness, efficiency, and usefulness of our solution.

==> images/experiments/Sensitivity/sigma/sigma_num.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[thick,xscale=0.575,yscale=0.45, every node/.style={transform shape}]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle \sigma\)},
xmin=0.9055, xmax=1.0045,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\# Maximal frequent node sets},
ymin=0.451385893609953, ymax=17967694.8589099,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
0.91 86
0.92 83
0.93 50
0.94 35
0.95 28
0.96 10
0.97 3
0.98 1
0.99 1
1 1
};
\addlegendentry{HomoSapiens}
\addplot [semithick, darkorange25512714, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0.91 410227
0.92 306724
0.93 148254
0.94 95073
0.95 32459
0.96 5542
0.97 514
0.98 410
0.99 32
1 1
};
\addlegendentry{Biomine}
\addplot [semithick, forestgreen4416044, mark=x, mark size=3, mark options={solid}]
table {%
0.91 8110364
0.92 1669133
0.93 1669133
0.94 298976
0.95 45243
0.96 8204
0.97 3555
0.98 514
0.99 94
1 1
};
\addlegendentry{Twitter}
\end{axis}

\end{tikzpicture}


==> images/experiments/Sensitivity/sigma/sigma_time.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[thick,xscale=0.575,yscale=0.45, every node/.style={transform shape}]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle \sigma\)},
xmin=0.9055, xmax=1.0045,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Running time (seconds)},
ymin=0.00633877479598292, ymax=2462.52437199995,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
0.91 0.0548341274261
0.92 0.0476040840149
0.93 0.0394289493561
0.94 0.0387048721313
0.95 0.0338761806488
0.96 0.0338299274445
0.97 0.0308990478516
0.98 0.0248048305511
0.99 0.0136420726776
1 0.0113780498505
};
\addlegendentry{HomoSapiens}
\addplot [semithick, darkorange25512714, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0.91 99.7155730724
0.92 68.344949007
0.93 23.2241790295
0.94 12.5043730736
0.95 2.9521279335
0.96 0.345778942108
0.97 0.0424509048462
0.98 0.030669927597
0.99 0.0194690227509
1 0.01740193367
};
\addlegendentry{Biomine}
\addplot [semithick, forestgreen4416044, mark=x, mark size=3, mark options={solid}]
table {%
0.91 1371.88601112
0.92 203.021579027
0.93 199.198103905
0.94 30.1536231041
0.95 3.41548109055
0.96 0.499230861664
0.97 0.173547029495
0.98 0.0369141101837
0.99 0.0300848484039
1 0.0280368328094
};
\addlegendentry{Twitter}
\end{axis}

\end{tikzpicture}


==> old/2-preliminaries_old.tex <==
\vspace{-1mm}
\section{Problems Formulation and Hardness}
\label{sec:preliminaries}
%
Let  $\mathcal{G} = (V,E,p)$ be a probabilistic (or uncertain), undirected, and unweighted graph, with the number of nodes $|V| = n$
and the number of edges $|E| = m$, where $E\subseteq V\times V$, and $p: E \rightarrow (0,1]$ is a function that assigns a probability of existence to each edge.
Following the majority of the literature on uncertain graphs \cite{V79,B86,PBGK10,KYC18,KBGN18,SahaBVKB21}, we adopt the well-established
{\em possible world} semantics and assume that the edges exist independent of each other. Therefore,
the uncertain graph $\mathcal{G}$ can be interpreted as a probability distribution over $2^{|E|}$ deterministic graphs (possible worlds)
$G=(V,E_G) \sqsubseteq \mathcal{G}$, obtained by sampling each edge $e \in E$ independently with probability $p(e)$.
The probability of a possible world $G=(V,E_G)$ being observed is:
%
\begin{align}
% \vspace{-3mm}
\small
\Pr(G)=\prod_{e\in E_G}p(e)\prod_{e\in E \setminus E_G}(1-p(e))
% \vspace{-3mm}
\end{align}
%
%Given a set $U \subseteq V$, the subgraph of $\mathcal{G}$ induced by $U$ is the uncertain graph $\mathcal{G}[U] = (U, E[U], p)$ where $E[U] = \{ (u, v) \in E : u \in U, v \in U \}$.
There are several notions of graph density in the context of a deterministic graph \cite{GT15,T15,FYCLX19}, such as
edge density, edge ratio, triangle density, clique density, pattern density, etc. We extend these definitions
over uncertain graphs as follows.
%
\subsection{Edge Density}
\label{sec:edge_density}
%
We first revisit the edge density in a deterministic graph.
%
\begin{defn}
[Edge Density \cite{G84}]
Given a deterministic graph $G = (V, E)$, the edge density (also known as the average degree) of $G$ is defined as:
%
\begin{equation}
    \small \rho(G) = \frac{|E|}{|V|}
\label{eq:edge_density}
\end{equation}
\label{def:edge_density}
\end{defn}
%
We now define the probability of an induced subgraph in an uncertain graph being a densest subgraph.
%
\begin{defn}
[Densest Subgraph Probability]
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and a node set $U \subseteq V$, the densest subgraph probability of $U$,
denoted by $\tau(U)$, is the sum of the probabilites of all possible worlds where the subgraph induced by $U$ has the largest edge density.
Formally,
%
\begin{equation}
    \small \tau(U) = \sum_{G \sqsubseteq \mathcal{G}} \Pr(G) \times \mathbbm{1} \left[ U = \argmax_{W \subseteq V} \rho(G[W]) \right]
\label{eq:densest_subgraph_probability}
\end{equation}
\label{def:densest_subgraph_probability}
\end{defn}
%
In the above equation, $G=(V,E_G) \sqsubseteq \mathcal{G}$ is a possible world, $W \subseteq V$, $G[W]= (W, E_G[W])$ denotes the subgraph of $G$ induced by $W$, where $E_G[W] = \{(u, v) \in E_G: u \in W, v \in W \}$. $\mathbbm{1} \left[ U = \argmax_{W \subseteq V} \rho(G[W]) \right]$ is an indicator function that returns 1 if the subgraph induced by $U$ has the largest edge density in $G$, and 0 otherwise. Note that the node set whose induced subgraphs have the maximum edge density in $G$ may not be unique.

Our goal is to find the node set which is the most likely to induce a densest subgraph in an uncertain graph, formally defined as follows.
%
\begin{problem}
[Most Probable Densest Subgraph (\textsf{MPDS})]
Given an uncertain graph $\mathcal{G} = (V, E, p)$, find the node set $U^* \subseteq V$ that has the highest densest subgraph probability. Formally,
\begin{equation}
    \small U^* = \argmax_{U \subseteq V} \tau(U)
\label{eq:mpds}
\end{equation}
\label{prob:mpds}
\end{problem}
%
\subsection{Clique Density}
\label{sec:clique_density}
%
We next extend our concept of edge density to clique density in uncertain graphs.
An $h$-clique is a complete graph of $h$ nodes, $h \ge$ 2. Notice that a 2-clique is an edge and a 3-clique denotes
a triangle. The $h$-clique densest subgraph problem aims at finding those subgraphs which are large near-cliques
rather than the subgraph that maximizes the average degree.
%
\begin{defn}
[$h$-Clique Density \cite{T15}]
Given a deterministic graph $G = (V, E)$ and an integer $h \geq 2$, the $h$-clique density of $G$ is defined as:
\begin{equation}
    \small \rho_h(G) = \frac{\mu_h(G)}{|V|}
\label{eq:clique_density}
\end{equation}
where $\mu_h(G)$ is the number of $h$-cliques in $G$.
\label{def:clique_density}
\end{defn}
%
\begin{defn}
[$h$-Clique Densest Subgraph Probability]
Given an uncertain graph $\mathcal{G} = (V, E, p)$, a node set $U \subseteq V$, and an integer $h \geq 2$, the $h$-clique densest subgraph probability of $U$, denoted by $\tau_h(U)$, is the sum of the probabilites of all possible worlds where the subgraph induced by $U$ has the largest $h$-clique density. Formally,
\begin{equation}
    \small \tau_h(U) = \sum_{G \sqsubseteq \mathcal{G}} \Pr(G) \times \mathbbm{1} \left[ U = \argmax_{W \subseteq V} \rho_h(G[W]) \right]
\label{eq:h_clique_densest_subgraph_probability}
\end{equation}
\label{def:h_clique_densest_subgraph_probability}
\end{defn}
%
\begin{figure}
  \centering
  \includegraphics[scale=0.27]{images/example/example2.jpg}
    \vspace{-3mm}
  \captionof{figure}{\small Clique density in an uncertain graph %\textcolor{olive}{\bf [AK: show up to $G_{10}$, five in each row.]}
  }
  \label{fig:example_2_clique}
    \vspace{-5mm}
\end{figure}
%
\begin{exam}
%\textcolor{olive}{\bf [AK: Show an example uncertain graph (could be different from Figure 1), some (e.g., 3) of its possible worlds and their existence probabilities.
%Show that in some of these possible worlds (e.g., 2), a node set induces a triangle-densest subgraph, whereas in others (e.g., 1) the same node set does not
%induce a triangle-densest subgraph.]}
Figure~\ref{fig:example_2_clique} shows an input uncertain graph and some of its possible worlds.
The subgraphs induced by the node set $\{A,C,D\}$ contain a 3-clique (i.e., triangle) only in possible worlds $G_1$, $G_2$, $G_3$, and $G_4$.
In fact, $\{A,C,D\}$ induces
3-clique densest subgraphs in possible worlds $G_1$, $G_2$, and $G_3$, thus the
3-clique densest subgraph probability of $\{A,C,D\}$ is 0.009 + 0.036 + 0.009 = 0.054.
%\textcolor{olive}{\bf [AK:...]}
%\textcolor{olive}{\bf [AK: make sure you can explain this with the shown possible worlds only, if not update which possible worlds must be shown.]}
\label{exam:clique}
\end{exam}
%
%
\begin{problem}
[Most Probable $h$-Clique Densest Subgraph (\textsf{$h$-Clique-MPDS})]
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and an integer $h \geq 2$, find the node set $U^* \subseteq V$ that has the highest $h$-clique densest subgraph probability. Formally,
\begin{equation}
    \small U^* = \argmax_{U \subseteq V} \tau_h(U)
    \label{eq:h_clique_mpds}
\end{equation}
\label{prob:h_clique_mpds}
\end{problem}
%
\subsection{Pattern Density}
\label{sec:pattern_density}
%
Our metric can also be generalized to pattern density in an uncertain graph.
Given an arbitrary pattern graph, the pattern density measures the average number of such pattern occurring in a subgraph.
%in which a node participates.
%
\begin{defn}
[Pattern Density \cite{FYCLX19}]
Given a deterministic graph $G = (V, E)$ and an input pattern graph $\psi$, the pattern density of $G$ with respect to $\psi$ is defined as:
\begin{equation}
    \small \rho_\psi(G) = \frac{\mu_\psi(G)}{|V|}
    \label{eq:pattern_density}
\end{equation}
where $\mu_\psi(G)$ is the number of instances of $\psi$ in $G$.
\label{def:pattern_density}
\end{defn}
%
\begin{defn}
[Pattern Densest Subgraph Probability]
Given an uncertain graph $\mathcal{G} = (V, E, p)$, a node set $U \subseteq V$, and an input pattern graph $\psi$, the pattern densest subgraph probability of $U$ with respect to $\psi$, denoted by $\tau_\psi(U)$, is the sum of the probabilites of all possible worlds where the subgraph induced by $U$ has the largest pattern density with respect to $\psi$. Formally,
\begin{equation}
    \small \tau_\psi(U) = \sum_{G \sqsubseteq \mathcal{G}} \Pr(G) \times \mathbbm{1} \left[ U = \argmax_{W \subseteq V} \rho_\psi(G[W]) \right]
    \label{eq:pattern_densest_subgraph_probability}
\end{equation}
\label{def:pattern_densest_subgraph_probability}
\end{defn}
%
\begin{figure}
  \centering
  \includegraphics[scale=0.27]{images/example/example3.jpg}
    \vspace{-3mm}
  \captionof{figure}{\small Pattern density (for a given pattern) in an uncertain graph %\textcolor{olive}{\bf [AK: show up to $G_{10}$, five in each row.]}
  }
  \label{fig:example_3_pattern}
    \vspace{-3mm}
\end{figure}
%
\begin{exam}
%\textcolor{olive}{\bf [AK: Show an example uncertain graph (same as Figure 2), some (e.g., 3) of its possible worlds and their existence probabilities.
%Show a small pattern (different from clique).
%Show that in some of these possible worlds (e.g., 2), a node set induces a pattern-densest subgraph, whereas in others (e.g., 1) the same node set does not
%induce a pattern-densest subgraph.]}
Figure~\ref{fig:example_3_pattern} shows an input uncertain graph, some of its possible worlds, and an input pattern graph ($\psi$). We notice that the subgraphs induced by node set $\{A,B,C,D\}$ contain $\psi$ only in possible worlds $G_2$, $G_3$, $G_4$, $G_5$, $G_6$, $G_7$, and $G_8$.
Moreover, $\{A,B,C,D\}$ induces the $\psi$-densest subgraphs in all these six possible worlds,
%\textcolor{olive}{\bf [AK:...]}
thus the $\psi$-densest subgraph probability of $\{A,B,C,D\}$ is 0.294.
%\textcolor{olive}{\bf [AK:...]}
%\textcolor{olive}{\bf [AK: make sure you can explain this with the shown possible worlds only, if not update which possible worlds must be shown.]} \textcolor{olive}{\bf [AK: the input uncertain graphs in Fig 2 and Fig 3 are same, but their possible world's are indexed differently, that is, $G_1$ is different in Fig 2 and 3. This will create confusion. It is better to use a structurally different, yet simple, uncertain graph in Fig 3.]}
\label{exam:motif}
\end{exam}
%
\begin{problem}
[Most Probable Pattern Densest Subgraph (\textsf{Pattern-MPDS})]
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and an input pattern graph $\psi$, find the node set $U^* \subseteq V$ that has the highest pattern densest subgraph probability with respect to $\psi$. Formally,
\begin{equation}
    \small U^* = \argmax_{U \subseteq V} \tau_\psi(U)
    \label{eq:pattern_mpds}
\end{equation}
\label{prob:pattern_mpds}
\end{problem}
%
\subsection{Further Extensions of Densest Subgraph Problems}
\label{sec:extention}
%
%
%\eat{
%Instead of the probability of a node set inducing {\em only} a densest subgraph, one may also be interested
%in a relaxed notion of the problem, such as the probability that the node set induces a reasonably dense subgraph
%(say, a subgraph with {\em at least} half the optimal density). This is formulated in the definition below.
%%
%\begin{defn}
%[Half-optimal Dense Subgraph Probability]
%Given an uncertain graph $\mathcal{G} = (V, E, p)$ and a node set $U \subseteq V$, the half-optimal dense subgraph probability of $U$,
%denoted by $\tau^{({\frac{1}{2}})}(U)$, is the sum of the probabilities of all possible worlds where the edge density of
%the subgraph induced by $U$ is at least half of the optimal subgraph edge density in that world. That is,
%%
%\begin{equation}
%    \small \tau^{({\frac{1}{2}})}(U) = \sum_{G \sqsubseteq \mathcal{G}} \Pr(G) \times \mathbbm{1} \left[ \rho(U) \geq \frac{1}{2} \max_{W \subseteq V} \rho(G[W]) \right]
%    \label{eq:half_optimal_dense_subgraph_probability}
%\end{equation}
%\label{def:half_optimal_dense_subgraph_probability}
%\end{defn}
%%
%The above definition is only for edge density; similar relaxations can also be made for clique and pattern densities.
%We now state the corresponding maximization problem.
%%
%\begin{problem}
%[Most Probable Half-optimal Dense Subgraph (\textsf{Half-Optimal-MPDS})]
%Given an uncertain graph $\mathcal{G} = (V, E, p)$, find the node set $U^* \subseteq V$ that has the highest half-optimal dense subgraph probability.
%Formally,
%\begin{equation}
%    \small U^* = \argmax_{U \subseteq V} \tau^{({\frac{1}{2}})}(U)
%    \label{eq:half_optimal_mpds}
%\end{equation}
%\label{prob:half_optimal_mpds}
%\end{problem}
%%
%}
%
\spara{Top-$k$ densest subgraphs.}
For each of the aforementioned notions of densest subgraphs, we define the problem of finding the top-$k$ node sets.
We only state the one for edge densest subgraphs below owing to space constraints.
%
\begin{problem}
[Top-$k$ Most Probable Densest Subgraph (\textsf{Top-$k$ MPDS})]
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and a positive integer $k$, find the top-$k$ distinct node sets $U_1^*, U_2^*, \ldots, U_k^*$,
where each $ U_i^* \subseteq V$, $i \leq k$, having the highest densest subgraph probabilities. Formally,
\begin{align}
   & \tau(U_i^*) \ge \tau(U_{i+1}^*) \quad \forall 1\leq i <k; \nonumber \\
   & \tau(U_i^*) \ge \tau(U) \quad \forall i \leq k \quad \text{and} \quad \forall U \subseteq V, \, U \not\in \{U_1^*, \ldots, U_k^*\}.
   %    \small \{U_1^*, \ldots, U_k^*\} = \argmax_{\{U_1, \ldots, U_k\} \subseteq 2^V} \sum_{i=1}^k \tau(U_i)
   \label{eq:top_k_mpds}
\end{align}
\label{prob:top_k_mpds}
\end{problem}
%

\spara{Nucleus densest subgraph.}
%\textcolor{olive}{\bf [AK: Say the motivation why we need this problem over large graphs, and how our new problem can resolve this issue. Then, formally
%state the problem.]}
In large-scale graphs, we observe that the densest subgraph probability of every node set can be quite small, adopting such node sets as {\sf MPDS} contradicts our goal of identifying node sets that can induce a densest subgraph with high probability.
%and thus computing the {\sf MPDS} might be less useful.
Instead, we find those node sets whose containment probability within a densest subgraph is higher than a user-input threshold. Such node sets form
the ``nucleus'' of various densest subgraphs across different possible worlds of the input uncertain graph.
%
\begin{defn}
[Densest Subgraph Containment Probability]
\label{def:pr}
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and a node set $U \subseteq V$, the densest subgraph containment probability of $U$, denoted by $\gamma(U)$, is the sum of the probabilities of all possible worlds $G$ such that $U$ is contained in a densest subgraph of $G$. Formally,
\begin{equation}
    \small \gamma(U) = \sum_{G \sqsubseteq \mathcal{G}} \Pr(G) \times \mathbbm{1} \left[ \exists \, U \subseteq U' \subseteq V \, : \, \tau(U') = \max_{V' \subseteq V} \tau(V') \right]
\end{equation}
\end{defn}
%
\begin{exam}
Considering the input uncertain graph in Figure~\ref{fig:example_1}, the node set $\{B,D\}$ can induce a densest subgraph with probability 0.42 (in possible worlds $G_4$ and $G_7$). We notice that $\{B,D\}$ is also likely to be contained in densest subgraphs of other possible worlds ($G_6$ and $G_8$),
even though $\{B,D\}$ alone does not induce a densest subgraph in these possible worlds. The overall densest subgraph containment probability of $\{B,D\}$ is 0.7 (due to possible worlds $G_4$, $G_6$, $G_7$, and $G_8$), which implies that this node set is a critical component in forming densest subgraphs.
%\textcolor{olive}{\bf [AK: Use the same uncertain graph as in Figure 1 or in Figure 2, consider a node set (more than 1 node)
%and show how its densest subgraph containment probability can be computed using the possible worlds shown earlier.]}
\label{exam:nucleus}
\end{exam}
%
\begin{problem}
[Nucleus Densest Subgraph (\textsf{NDS})]
\label{prob:cont_min}
Given an uncertain graph $\mathcal{G} = (V, E, p)$ and an input probability threshold $\sigma$,
find all node sets whose densest subgraph containment probability is at least $\sigma$, i.e., \begin{equation}
    \small \mathcal{U} = \left\{ U \subseteq V : \gamma(U) \geq \sigma \right\}
\end{equation}
\end{problem}
%
Notice that the {\sf NDS} problem can be analogously extended to {\sf $h$-Clique-NDS} and {\sf Pattern-NDS} problems.
%

\spara{Remarks.}
\textcolor{red}{[AK: A similar comment like our InfoVote paper would be that we have too many problem definitions. We must state here briefly
when to use what.]}
%
\subsection{Hardness}
\label{sec:hardness}
%
Our problems are challenging since computing the densest subgraph probability of a given node set is $\sharpP$-hard.
%
\begin{theor}
\label{th:hard}
Given an uncertain graph $G = (V, E, p)$ and a node set $U \subseteq V$, computing the densest subgraph probability of $U$ is $\sharpP$-hard.
\end{theor}
%
\begin{proof}
We prove by a reduction from the $\sharpP$-hard problem of finding the number of matchings in a graph \cite{V79}. A matching in a deterministic graph $G = (V, E)$ is an edge
set $M \subseteq E$ without any common nodes.

Consider a deterministic graph $G = (V, E)$. This graph is transformed, by adding two new nodes $v_1$ and $v_2$ along with an edge between them, into an uncertain graph $\mathcal{G} = (V \cup \{v_1, v_2\}, E \cup \{(v_1, v_2)\}, p)$, where the probability of each edge is $0.5$, except the new edge $(v_1, v_2)$ which has probability 1. Clearly, this reduction takes $\bigO(|E|)$ time, which is polynomial in the size of $G$. It can be shown that:
\begin{itemize}
    \item Any possible world $G' \sqsubseteq \mathcal{G}$ with non-zero probability has $\Pr(G') = (0.5)^{|E|}$.
    \item There is a bijection between the set of subsets of $E$ and the set of possible worlds of $\mathcal{G}$ with non-zero probability.
    \item The node set $\{v_1, v_2\}$ induces a densest subgraph in a possible world if and only if every node has degree at most 1 in that world, i.e., the edges in the world excluding $(v_1, v_2)$ form a matching in $G$.
\end{itemize}

Hence, we have:
\begin{small}
\begin{align*}
    &\tau(\{v_1, v_2\}) = \sum_{G' \sqsubseteq \mathcal{G}} \Pr(G') \times \mathbbm{1} \left[ \{v_1, v_2\} = \argmax_{W \subseteq V} \rho(G'[W]) \right] \\
    &= \sum_{G' \sqsubseteq \mathcal{G}} \Pr(G') \times \mathbbm{1} \left[ \text{each node has degree at most 1 in }G' \right] \\
    &= (0.5)^{|E|} \sum_{G' \sqsubseteq \mathcal{G} : \Pr(G') \neq 0}\!\!\!\!\!\! \mathbbm{1} \left[ \text{each node has degree at most 1 in }G' \right] \\
    &= (0.5)^{|E|} \sum_{M \subseteq E} \mathbbm{1} \left[ \text{M is a matching in $G$} \right]
\end{align*}
\end{small}
%
The sum in the last line above is the number of matchings in $G$. Thus, a solution to our problem on $\mathcal{G}$ provides a solution to the matching counting problem on $G$.
\end{proof}
%
Since the computation of $\tau(U)$, for a given $U$, is $\sharpP$-hard, the computations of its generalizations $\tau_h(U)$ and $\tau_\psi(U)$ are also $\sharpP$-hard.
Thus, finding the node sets with the top-$k$ densest subgraph probabilities, as well as computing the {\sf NDS} are also very difficult.
{\em Given such computational challenges, we design approximate algorithms, with end-to-end accuracy guarantees, to find the most-probable densest subgraphs in an uncertain graph, based on various graph density notions}.   

==> old/3-exact_old.tex <==
\section{Approximate Solutions for Densest Subgraphs}
\label{sec:mpds_algo}
In this section, we describe our methods for approximating the top-$k$ subgraphs having the highest densest subgraph probabilities,
along with end-to-end theoretical accuracy guarantees.
%, for each notion of density: edge (\S~\ref{sec:top_k_mpds_algorithm}), clique (\S~\ref{sec:clique}), and pattern (\S~\ref{sec:pattern}).
Our {\bf technical contributions} include the following: {\bf (1)} We {\em design novel approximation algorithms, with end-to-end accuracy guarantees, for computing the most probable densest subgraph in an uncertain graph for all notions of density: edge (\S~\ref{sec:top_k_mpds_algorithm}), clique (\S~\ref{sec:clique}), pattern (\S~\ref{sec:pattern})}.
{\bf (2)} As building blocks of the algorithms for clique and pattern densities, we also {\em design novel methods to compute all clique and pattern densest subgraphs
in a deterministic graph}.
%(Although the methods are similar to \cite{CQ20}, which computes all edge densest subgraphs, not all definitions and proofs in \cite{CQ20} can be extended trivially to clique and pattern densities.)
{\bf (3)}  Additionally, we use these methods to {\em design approximation algorithms, with theoretical quality guarantees,
for computing the corresponding nucleus densest subgraphs (\S~\ref{sec:nucleus})}.% \textcolor{olive}{\bf [AK: elaborate]}
%
\subsection{\textsf{Top-$k$ MPDS}: Approximate Algorithm}
\label{sec:top_k_mpds_algorithm}
%
\begin{algorithm}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\scriptsize
	\caption{\small Estimate the \textsf{Top-$k$ MPDS} in an uncertain graph} \label{alg:exact}
	\begin{algorithmic}[1]
		\REQUIRE Uncertain graph $\mathcal{G} = (V,E,p)$, positive integer $k$, and number of samples $\theta$
		\ENSURE (Approximate) \textsf{Top-$k$ MPDS}
		\FORALL{$U \subseteq V$}
		\STATE $\widehat{\tau}(U) \gets 0$
		\ENDFOR
		\FOR{$i = 1$ \TO $\theta$}
		\STATE Sample a possible world $G \sqsubseteq \mathcal{G}$
		\STATE $S \gets $ All densest subgraphs in $G$ via \cite{CQ20} \label{line:all_densest}
		\FORALL{$U \in S$}
		\STATE $\widehat{\tau}(U) \gets \widehat{\tau}(U) + \frac{1}{\theta}$
		\ENDFOR
		\ENDFOR
		\RETURN Top-$k$ $U$'s having the highest $\widehat{\tau}(U)$ %$\argmax_{\{U_1, \ldots, U_k\} \subseteq 2^V} \sum_{i=1}^k \widehat{\tau}(U_i)$
	\end{algorithmic}
\end{algorithm}

The proposed solution (Algorithm \ref{alg:exact}) runs $\theta$ independent
iterations as follows: Sample a possible world $G \sqsubseteq \mathcal{G}$ and find {\em all} the node sets
inducing the densest subgraphs in $G$ (Line \ref{line:all_densest}).
Denoting by $\widehat{\tau}(U)$ the average frequency (across $\theta$ rounds) of a node set $U$
inducing a densest subgraph, the top-$k$ node sets finally returned are the ones that have the highest estimated densest subgraph probabilities $\widehat{\tau}(U)$.

We apply the technique in \cite{CQ20} to compute all densest subgraphs in a deterministic graph (Line \ref{line:all_densest}). It involves reducing the graph to its $\lceil \Tilde{\rho} \rceil$-core \cite{BZ03}, where $\Tilde{\rho}$ is a lower bound on the
maximum edge density $\rho^*$ of any subgraph. This is followed by computing $\rho^*$ using the
state-of-the-art Goldberg's algorithm \cite{G84}. During each iteration of its binary search, the Goldberg's algorithm tries to find a subgraph with density larger than a guessed value $\alpha$ by computing the minimum cut in a flow network parameterized by $\alpha$.
Once $\rho^*$ is found, all densest subgraphs are enumerated by
traversing the strongly connected components (SCCs) in the residual graph (under a maximum flow)
of the flow network with $\alpha = \rho^*$; the details can be found in \cite{CQ20} and in the example below.
%
\begin{exam}
We compute all densest subgraphs in a possible world $G$ (Figure~\ref{fig:example_5_edge}(b)) of an uncertain graph $\mathcal{G}$ ((Figure~\ref{fig:example_5_edge}(a)). A flow network $G_{\alpha}$ (Figure~\ref{fig:example_5_edge}(c)) is constructed as follows. (1) Add a source node $s$ and a target node $t$. (2) If edge $(u,v)$ exists in $G$, add an edge from $u$ to $v$ and one from $v$ to $u$ in $G_{\alpha}$, both with capacity 1. (3) Add an edge from $s$ to each node $v$ in $G$ with capacity equal to the degree of $v$ in $G$. (4) Add and edge from each node in $G$ to $t$ with capacity $2\alpha$. Goldberg's algorithm \cite{G84} conducts a binary search with $[0,m]$ as the initial range of $\alpha$. In each iteration, it guesses an $\alpha$ and computes the maximum flow (minimum cut) in the flow network.
%\textcolor{olive}{[COMMENT AK: What is $m$? no of edges in $G$ or in $\mathcal{G}$?]}
Once terminated, %(the range size is smaller than $\frac{1}{n(n-1)}$), \textcolor{olive}{[Do we need to specify range size when terminated?]}
the optimal density is assigned to be $\rho^*=\alpha$.
In this example, we get $\rho^*=1$ and a densest subgraph $\{A,B,C,D\}$ (which corresponds to the minimum cut).
To find the other densest subgraphs, we create the residual graph ((Figure~\ref{fig:example_5_edge}(d)) by removing all the edges with zero residual capacity.
We enumerate the densest subgraphs by exploring the SCCs in this residual graph. In this case, we find one additional densest subgraph $\{B,C,D\}$.
\label{example:edge_density_flow}
%\textcolor{olive}{\bf [AK: add a running example for Algorithm \ref{alg:exact}. In particular, show an uncertain graph, a possible world of it that contains more than one (e.g., two) densest subgraphs, and show how they can be computed in Line \ref{line:all_densest} of Algorithm \ref{alg:exact}.]}
\end{exam}
%
\spara{Space complexity.} The majority of the memory is consumed by the flow network in each iteration of
the binary search, and hence the overall space complexity is $\bigO(m + n)$.

\begin{figure}
  \centering
  \includegraphics[scale=0.35]{images/example/example5.jpg}
    \vspace{-2mm}
  \captionof{figure}{\small Finding all densest subgraphs in a deterministic instance
  }
  \label{fig:example_5_edge}
    \vspace{-5mm}
\end{figure}

\spara{Time complexity.} The computation of the $\lceil \Tilde{\rho} \rceil$-core takes $\bigO(m)$ time \cite{BZ03}. Let $n_c$ and $m_c$ denote the number of nodes and edges respectively in the $\lceil \Tilde{\rho} \rceil$-core of a sampled possible world $G \sqsubseteq \mathcal{G}$. As shown in \cite{CQ20},
the computation of $\rho^*$ takes $\bigO \left( n_c m_c \log \left( \frac{n_c^2}{m_c} \right) \right)$ time,
while the enumeration of the densest subgraphs takes $\bigO(L)$ time per subgraph, where $L$ is the
number of nodes in that densest subgraph (note that $L \leq n$). Denoting respectively by $n_c^*$, $m_c^*$, $d^*$
and $L^*$ the maximum number of nodes, edges, densest subgraphs and nodes in a densest subgraph
in any possible world, the overall time complexity of our algorithm is
$\bigO \left( \theta \left( m + n_c^* m_c^* \log \left( \frac{n_c^{*2}}{m_c^*} \right) + d^*L^* \right) \right)$.
Practically, $n_c^* \ll n$ and $m_c^* \ll m$, as validated in our experiments (\S~\ref{sec:exp}).
For instance, $\frac{n_c^*}{n}$ = \textcolor{olive}{0.XX}, $\frac{L^*}{n}$ = \textcolor{olive}{0.XX},
$\frac{m_c^*}{m}$ = \textcolor{olive}{0.YY}, and $d^*$ = \textcolor{olive}{WW}
in our largest \textcolor{olive}{ZZ} dataset, making Algorithm~\ref{alg:exact} efficient even with large-scale graphs.

\textcolor{red}{discussion on $\theta$ and other sampling method.}
% We would like $\theta$ to be large enough to ensure that, with a high probability, the estimate $\widehat{\rho}(U)$ is very close to $\rho(U)$ for each $U \subseteq V$. This is shown in the theorem below.

% \begin{theor}
% Given $\epsilon, \delta > 0$, suppose $\theta$ satisfies
% \begin{equation}
%     \small \theta \geq \frac{(n + 1) \ln 2 - \ln \delta}{2\epsilon^2} \label{eq:theta}
% \end{equation}
% Then $\left| \widehat{\rho}(U) - \rho(U) \right| < \epsilon$ for all node sets $U \subseteq V$ with probability at least $1 - \delta$.
% \begin{proof}
% Using the union bound and Hoeffding's inequality, %we have
% \begin{small}
% \begin{align*}
%     &\Pr \left( \forall U \subseteq V : \left| \widehat{\rho}(U) - \rho(U) \right| < \epsilon \right) \\
%     &= 1 - \Pr \left( \exists U \subseteq V : \left| \widehat{\rho}(U) - \rho(U) \right| \geq \epsilon \right) \\
%     &\geq 1 - \sum_{U \subseteq V} \Pr \left( \left| \widehat{\rho}(U) - \rho(U) \right| \geq \epsilon \right) \\
%     &\geq 1 - 2^n \cdot 2 \exp \left( -2\theta\epsilon^2 \right) \\
%     &\geq 1 - \delta
% \end{align*}
% \end{small}
% \end{proof}
% \end{theor}

\spara{Accuracy guarantee.} We prove that,
with a high probability, our algorithm returns the true top-$k$ node sets.
We first ensure that with a high probability,
the true top-$k$ node sets are included as candidate node sets
\footnote{\scriptsize{A node set $U$ is called a candidate node set if its estimated probability $\widehat{\tau}(U)>0$ after
$\theta$ rounds, indicating that $U$ induces a densest subgraph in at least one of these $\theta$ possible worlds of $\mathcal{G}$.}}
after $\theta$ rounds,
and then we ensure that those sets are indeed the ones having the $k$ largest estimated probabilities, presented as Theorems \ref{th:cv} and \ref{th:topk}, respectively.

\begin{theor}
Let $V_1, \ldots, V_{k}$ denote the true top-$k$ node sets, and let $CV$ denote the set of candidate node sets after $\theta$ rounds. Then,
\begin{equation}
    \small \Pr \left( \left\{V_1, \ldots, V_k \right\} \subseteq CV \right) \geq 1 - \sum_{i=1}^k \left( 1 - \tau(V_i) \right)^\theta
    \label{eq:cv}
\end{equation}
\label{th:cv}
\end{theor}
%
\begin{proof}
From the union bound, we have:
\begin{footnotesize}
\begin{align*}
    &\Pr \left( \left\{V_1, \ldots, V_k \right\} \subseteq CV \right)
    % = \Pr \left( \bigwedge_{i=1}^k V_i \in CV \right)
    = 1 - \Pr \left( \bigvee_{i=1}^k V_i \notin CV \right) \\
    & \geq 1 - \sum_{i=1}^k \Pr \left( V_i \notin CV \right) = 1 - \sum_{i=1}^k \left( 1 - \tau(V_i) \right)^\theta
    % &= \sum_{i=0}^k (-1)^i \sum_{S \subseteq \left\{V_1, \ldots, V_k \right\} : |S| = i} \left( 1 - \sum_{U \in S} \rho(U) \right)^\theta
\end{align*}
\end{footnotesize}
\end{proof}
%
% \textcolor{olive}{\bf [AK: give intuition why the above is a good result.]}
From Theorem \ref{th:cv}, if the true top-$k$ densest subgraph probabilities and the number of sampled possible worlds are reasonably large, then the true top-$k$ node sets are all included in the candidate node set with a high probability, which is necessary if all of them are to be the ones finally returned by our algorithm.

\begin{lem}
$\widehat{\tau}(U)$ is an unbiased estimate of $\tau(U)$. Formally, $\mathbbm{E}[\widehat{\tau}(U)] = \tau(U)$.
\end{lem}
\begin{proof}
Let $X_i(U)$ be a binary random variable denoting whether $U$ induces a densest subgraph in the $i^{th}$ possible world; thus $\widehat{\tau}(U) = \frac{1}{\theta} \sum_{i=1}^\theta X_i(U)$. Clearly, $\mathbbm{E}[X_i(U)] = \Pr \left( X_i[U] = 1 \right) = \tau(U)$, and hence $\mathbbm{E}[\widehat{\tau}(U)] = \tau(U)$.
\end{proof}
% \textcolor{olive}{\bf [AK: make it a lemma and state its importance.]}
The unbiasedness of $\widehat{\tau}(U)$ is useful because it ensures that, as the number of samples $\theta$ increases, the estimate $\widehat{\tau}(U)$ goes closer to the true value $\tau(U)$.
%
\begin{theor}
Let $V_1, \ldots, V_{k+1}$ denote the true top-$(k+1)$ node sets, and let $CV$ denote the set of candidate node sets after $\theta$ rounds. Define $mid = \frac{1}{2} \left[ \tau\left(V_k\right) + \tau\left(V_{k+1}\right) \right]$ and
\begin{equation}
    \small
    d_U =
    \begin{cases}
    \tau(U) - mid & \text{if} \, \, U \in \{V_1, \ldots, V_k\} \\
    mid - \tau(U) & \text{otherwise}
    \end{cases}
\end{equation}
% Suppose $\theta$ satisfies \eqref{eq:theta}.
Then, the probability that $V_1, \ldots, V_k$ are returned by Algorithm~\ref{alg:exact} is at least
\begin{equation}
    % \small \left[ 1 - \sum_{i=1}^k \left( 1 - \rho(V_i) \right)^\frac{(n + 1) \ln 2 - \ln \delta}{2\epsilon^2} \right] \left[ 1 - \sum_{U \in CV} \left( \frac{\delta}{2^{n+1}} \right)^{\left( \frac{d_U}{\epsilon} \right)^2} \right]
    \small \left[ 1 - \sum_{i=1}^k \left( 1 - \tau(V_i) \right)^\theta \right] \left[ 1 - \sum_{U \in CV} \exp \left( -2d_U^2\theta \right) \right] \label{eq:prf}
\end{equation}
\label{th:topk}
\end{theor}
%
\begin{proof}
We have:
\begin{footnotesize}
\begin{align}
    &\Pr(V_1, \ldots V_k \text{ are returned}) \geq \Pr(\{V_1, \ldots, V_k\} \subseteq CV) \times \nonumber \\
    &\quad \Pr \left( \bigwedge_{U \in \{V_1, \ldots, V_k\}} \!\!\!\!\!\! \widehat{\tau}(U) > mid \wedge \bigwedge_{U \in CV \setminus \{V_1, \ldots, V_k\}} \!\!\!\!\!\! \widehat{\tau}(U) < mid \right) \label{eq:pr1}
\end{align}
\end{footnotesize}
Now, using the union bound and Hoeffding's inequality,
\begin{footnotesize}
\begin{align}
    &\Pr \left( \bigwedge_{U \in \{V_1, \ldots, V_k\}} \widehat{\tau}(U) > mid \wedge \bigwedge_{U \in CV \setminus \{V_1, \ldots, V_k\}} \widehat{\tau}(U) < mid \right) \nonumber \\
    &= 1 - \Pr \left( \bigvee_{U \in \{V_1, \ldots, V_k\}} \!\!\!\!\!\! \widehat{\tau}(U) \leq mid \vee \bigvee_{U \in CV \setminus \{V_1, \ldots, V_k\}} \!\!\!\!\!\! \widehat{\tau}(U) \geq mid \right) \nonumber \\
    &\geq 1 - \sum_{U \in \{V_1, \ldots, V_k\}} \!\!\!\!\!\! \Pr \left( \widehat{\tau}(U) \leq mid \right) - \sum_{U \in CV \setminus \{V_1, \ldots, V_k\}} \!\!\!\!\!\!\!\!\! \Pr \left( \widehat{\tau}(U) \geq mid \right) \nonumber \\
    % &= 1 - \sum_{U \in \{V_1, \ldots, V_k\}}\!\!\!\!\!\!\!\!\!\!\!\! \Pr \left( \widehat{\tau}(U) - \tau(U) \leq -d_U \right) - \sum_{U \in CV \setminus \{V_1, \ldots, V_k\}}\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \Pr \left( \widehat{\tau}(U) - \tau(U) \geq d_U \right) \nonumber \\
    &= 1 - \sum_{U \in \{V_1, \ldots, V_k\}} \Pr \left( \widehat{\tau}(U) - \tau(U) \leq -d_U \right) \nonumber \\
    &\qquad - \sum_{U \in CV \setminus \{V_1, \ldots, V_k\}} \Pr \left( \widehat{\tau}(U) - \tau(U) \geq d_U \right) \nonumber \\
    &\geq 1 - \sum_{U \in CV} \exp \left( -2d_U^2\theta \right) \label{eq:pr2}
\end{align}
\end{footnotesize}
Finally, plugging \eqref{eq:cv} and \eqref{eq:pr2} into \eqref{eq:pr1}, we obtain \eqref{eq:prf}.
% \begin{footnotesize}
% \begin{align*}
%     &\Pr(V_1, \ldots V_k \text{ are returned}) \\
%     &\geq \Pr(\{V_1, \ldots, V_k\} \subseteq CV) \times \left[ 1 - \sum_{U \in CV} \exp \left( -2d_U^2\theta \right) \right] \\
%     &\geq \left[ 1 - \sum_{i=1}^k \left( 1 - \tau(V_i) \right)^\theta \right] \left[ 1 - \sum_{U \in CV} \exp \left( -2d_U^2\theta \right) \right]
%     % &\geq \left[ 1 - \sum_{i=1}^k \left( 1 - \rho(V_i) \right)^\frac{(n + 1) \ln 2 - \ln \delta}{2\epsilon^2} \right] \left[ 1 - \sum_{U \in CV} \left( \frac{\delta}{2^{n+1}} \right)^{\left( \frac{d_U}{\epsilon} \right)^2} \right]
% \end{align*}
% \end{footnotesize}
\end{proof}
%
% \textcolor{olive}{\bf [AK: fix column overrun. Give intuition why the above is a good result.]}

From Theorem \ref{th:topk}, if the true top-$k$ densest subgraph probabilities are reasonably large and such probabilities
for other subgraphs are reasonably smaller (which is usually the case in our medium-size real-world uncertain graph datasets),
and if the number of sampled possible worlds ($\theta$) is sufficiently large,
then the true top-$k$ node sets are the ones finally returned by Algorithm \ref{alg:exact} with a high probability.


\input{3b-clique}


\input{3c-pattern} 

==> old/3b-clique_old.tex <==
\subsection{\textsf{$h$-Clique-MPDS}: Approximate Algorithm}
\label{sec:clique}

The algorithmic framework and accuracy guarantees remain the same as in \S \ref{sec:top_k_mpds_algorithm}, except that in Line \ref{line:all_densest} of Algorithm \ref{alg:exact}, we need to find {\em all} clique-densest subgraphs of the sampled possible world $G$. Inspired by \cite{MPPTX15, FYCLX19, CQ20}, we develop a novel, exact, and efficient solution, as shown in Algorithm \ref{alg:clique_densest}. Recall that {\em the problem of finding all clique-densest subgraphs in a deterministic graph itself is a novel problem, and none of
\cite{MPPTX15, FYCLX19, CQ20} studied this problem. Therefore, Algorithm \ref{alg:clique_densest} is one of our novel technical contributions}.

Algorithm \ref{alg:clique_densest} consists of two general steps. First, it applies the technique in \cite{FYCLX19} to compute the maximum density of any subgraph of $G$. Then, a suitable flow network $\mathcal{H}$ is constructed following \cite{MPPTX15, CQ20}. The SCCs of the residual graph under a maximum flow in $\mathcal{H}$ indicate all densest subgraphs of $G$. A more detailed walk-through of our approach is provided below.
%
\begin{algorithm}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\scriptsize
	\caption{\small Find all clique-densest subgraphs} \label{alg:clique_densest}
	\begin{algorithmic}[1]
		\REQUIRE Deterministic graph $G = (V,E)$, positive integer $h$
		\ENSURE All $h$-clique densest subgraphs in $G$
		\STATE $\Tilde{\rho} \gets $ Density returned by the peeling method \cite{T15, FYCLX19} \label{line:lb}
		\STATE $G \gets (\lceil \Tilde{\rho} \rceil, h)$-core of $G$ \cite{FYCLX19} \label{line:core}
		\STATE $\Lambda \gets $ All $(h-1)$-cliques contained in $h$-cliques in $G$ \label{line:all_instance}
		\STATE $\rho_h^* \gets \max_{S \subseteq V} \rho_h(S)$ \cite{SDCS20} \label{line:val}
		\STATE $\mathcal{H} \gets $ Alg. \ref{alg:flow} ($G$, $\Lambda$, $\rho_h^*$) \cite{MPPTX15, FYCLX19} \label{line:begin_enum_all}
		\STATE $f^* \gets $ Maximum flow in $\mathcal{H}$ \label{line:max_flow}
		\STATE $\mathcal{C} \gets $ SCCs of the residual graph $\mathcal{H}_{f^*}$, excluding those of $s$ and $t$ \label{line:scc}
		\RETURN Alg. \ref{alg:enum} ($\emptyset$, $\mathcal{C}$, $V$) \label{line:end_enum_all}
	\end{algorithmic}
\end{algorithm}

First, we define the clique degree (Definition \ref{def:clique_deg}) and the clique-based core (Definition \ref{def:core}) in a deterministic graph.

\begin{defn}
[$h$-Clique Degree \cite{FYCLX19}]
\label{def:clique_deg}
Given a deterministic graph $G$, a node $v$ and a positive integer $h$, the $h$-clique degree of $v$ in $G$, denoted by $deg_G(v, h)$, is the number of $h$-cliques in $G$ which contain $v$.
\end{defn}

\begin{defn}
[$(k, h)$-Core \cite{FYCLX19}]
\label{def:core}
Given a deterministic graph $G$ and two integers $h > 0$ and $k \geq 0$, the $(k, h)$-core of $G$, denoted by $\mathcal{R}_k$, is the largest subgraph of $G$ such that, for every node $v$ in $\mathcal{R}_k$, $deg_{\mathcal{R}_k} (v, h) \geq k$.
\end{defn}

Armed with these definitions, we proceed to the details of Algorithm \ref{alg:clique_densest}.
% \textcolor{olive}{\bf [AK: Algorithm \ref{alg:clique_densest} has three broad steps, which are given in three paragraphs below. First give an overview of these three steps and some intuition how those lead to the final correct solution. Then, give Line-wise explanation as below.]}
First, in Line \ref{line:lb}, it runs the peeling method of \cite{T15}, which iteratively removes the node with the smallest $h$-clique degree and returns the maximum density among all the resultant subgraphs, denoted by $\Tilde{\rho}$. Then, in Line \ref{line:core}, it replaces $G$ with its $(\lceil \Tilde{\rho} \rceil, h)$-core, i.e., the subgraph induced by those nodes which have $h$-clique degree at least $\Tilde{\rho}$. After that, Line \ref{line:all_instance} computes the set $\Lambda$ of all $(h-1)$-cliques contained in $h$-cliques in $G$, which are enumerated using the method in \cite{DBS18}. Line \ref{line:val} computes $\rho_h^*$, the maximum $h$-clique density of any subgraph, by the method in \cite{SDCS20}, which iteratively computes a (predicted) clique-densest subgraph via optimizing a convex program. The iterations stop once the computed subgraph is deemed to be indeed clique-densest, which is tested by means of an improved version of the Goldberg's condition \cite{G84} stating that the densities of two subgraphs cannot be ``too close'', or by checking if the maximum flow in a suitable flow network is the largest possible. After that, the clique-density of the computed subgraph is returned.
% conducts a binary search over the possible values $\alpha$ of $\rho_h^*$ and, for each $\alpha$, it computes the minimum cut in a suitable flow network to decide whether the true value of $\rho_h^*$ is greater or smaller than $\alpha$.

Once $\rho_h^*$ is obtained, Lines \ref{line:begin_enum_all}-\ref{line:end_enum_all} of Algorithm \ref{alg:clique_densest} enumerate all $h$-clique densest subgraphs of $G$. Line \ref{line:begin_enum_all} uses the method in \cite{MPPTX15, FYCLX19} to construct a flow network $\mathcal{H}$ which, briefly speaking, contains one node for each $(h-1)$-clique in $\Lambda$ and one for each node in $V$, in addition to a source node $S$ and a sink node $T$; the pseudocode is included in Appendix \ref{sec:clique_proof}. Once $\mathcal{H}$ is constructed, Algorithm \ref{alg:clique_densest} computes a maximum flow $f^*$ in $\mathcal{H}$ (Line \ref{line:max_flow}) and then identifies the strongly connected components (SCCs) of the residual graph $\mathcal{H}_{f^*}$ of $\mathcal{H}$ under $f^*$ (edges with zero residual capacity are removed).

Finally, in Line \ref{line:end_enum_all}, Algorithm \ref{alg:enum} is applied to extract all densest subgraphs of $G$. At a high level, Algorithm \ref{alg:enum} enumerates one densest subgraph of $G$ for every value of $C \cup des(C)$, where $C$ is an SCC of $\mathcal{H}_{f^*}$, and the set $des(C)$ (resp. $anc(C)$) denotes the set of SCCs having a directed path from (resp. to) $C$ in the SCC graph of $\mathcal{H}_{f^*}$. The detailed theoretical analyses for Algorithms \ref{alg:clique_densest}-\ref{alg:enum} are given in Appendix \ref{sec:clique_proof}.
%
\begin{figure}
  \centering
  \includegraphics[scale=0.31]{images/example/example6.jpg}
   \vspace{-2mm}
  \captionof{figure}{\small Finding all $h$-clique densest subgraphs in a deterministic instance ($h=3$)
  }
  \label{fig:example_6_clique}
    \vspace{-5mm}
\end{figure}

\begin{exam}
We compute all $h$-clique densest subgraphs ($h = 3$) in a possible world $G$ (Figure~\ref{fig:example_6_clique}(b)) of an uncertain graph $\mathcal{G}$ ((Figure~\ref{fig:example_6_clique}(a)). The maximum 3-clique density $\rho_h^*$ of any subgraph of $G$ can be easily computed as $\frac{1}{3}$. A flow network $G_{\alpha}$ is constructed as in Figure~\ref{fig:example_6_clique}(c). Instead of directly adding edges between nodes like for edge density (Example~\ref{example:edge_density_flow}), a new set of nodes representing the $(h-1)$-cliques is added. A $(h-1)$-clique node $\psi_i$ has a directed edge to each node contained in this $(h-1)$-clique, with infinite capacity. If a node $v$ forms an $h$-clique with the $(h-1)$-clique $\psi_i$, a directed edge from $v$ to $\psi_i$ is added with capacity 1. For simplicity, we only mark the capacities for the edges entering and leaving $\psi_1$ in Figure~\ref{fig:example_6_clique}(c). In this example, the $(h-1)$-cliques are all edges in the possible world, as shown in Figure~\ref{fig:example_6_clique}(d). After plugging in the maximum 3-clique density $\rho_h^*=\frac{1}{3}$ and computing the maximum flow, we identify a 3-clique densest subgraph $\{A,B,C,D,E,F\}$, and obtain a residual graph as shown in Figure~\ref{fig:example_6_clique}(e). The remaining 3-clique densest subgraphs are $\{A,B,C\}$ and $\{D,E,F\}$. Each of them corresponds to an SCC of the residual graph.
%\textcolor{olive}{\bf [AK: add a running example of all the steps, in particular, the example should demonstrate Lines \ref{line:begin_enum_all}-\ref{line:end_enum_all} of Algorithm \ref{alg:clique_densest}, assuming $\rho_h^*$ has been computed. Also, highlight the differences w.r.t. Example 5.]}
\label{exam:clique_densest}
\end{exam}
%
% \textcolor{olive}{\bf [AK: add a remark paragraph to say the novelty w.r.t. \cite{CQ20}. Why \cite{CQ20} can be extended for clique problem, yet it is novel?]}
\spara{Remark.} Our Algorithm \ref{alg:clique_densest} for computing all clique-densest subgraphs has similarities
to the method of computing all edge-densest subgraphs in \cite{CQ20}.
{\em However, there are also major differences from \cite{CQ20}, as demonstrated in Example \ref{exam:clique_densest}. Therefore,
the correctness of our method does not follow trivially from \cite{CQ20}}.
This is because our flow network $\mathcal{H}$ is different; it has one node for each $(h-1)$-clique in $\Lambda$ (in addition to one for each node in $V$ as in \cite{CQ20}), and the edges are from nodes in $V$ to nodes in $\Lambda$ (unlike \cite{CQ20}, where the edges are between nodes in $V$). Thus, as detailed in Appendix \ref{sec:clique_proof}, some non-trivial additions need to be incorporated into the definitions and proofs in \cite{CQ20} to prove the correctness of our Algorithms \ref{alg:clique_densest}-\ref{alg:enum}. {\em This forms one of our novel technical contributions}.
%
\begin{algorithm}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\scriptsize
	\caption{\small Enumerate all clique densest subgraphs} \label{alg:enum}
	\begin{algorithmic}[1]
		\REQUIRE Component sets $\mathcal{C}_1$ and $\mathcal{C}_2$, node set $V$
		\ENSURE All clique-densest subgraphs
		\STATE $R \gets \emptyset$
		\IF{$\mathcal{C}_1 \neq \emptyset$}
		\STATE $R \gets R \cup \left( \bigcup_{C \in \mathcal{C}_1 \cup des(\mathcal{C}_1)} C \cap V \right)$
		\ENDIF
		\FORALL{$C \in \mathcal{C}_2$}
		\IF{$C \cap V \neq \emptyset$}
		\STATE $\mathcal{C}_2 \gets \mathcal{C}_2 \setminus \{C\}$ \label{line:rem}
		\STATE $S \gets $ Alg. \ref{alg:enum} ($\mathcal{C}_1 \cup \{C\}$, $\mathcal{C}_2 \setminus (des(C) \cup anc(C))$, $V$) \label{line:rec}
		\STATE $R \gets R \cup S$
		\ENDIF
		\ENDFOR
		\RETURN $R$
	\end{algorithmic}
\end{algorithm}

\spara{Space complexity.} Let $G_c$ be the $(\lceil \Tilde{\rho} \rceil, h)$-core in Lines \ref{line:lb}-\ref{line:core} of Algorithm \ref{alg:clique_densest}, with $n_c$ and $m_c$ the corresponding node and edge counts, respectively. As each $h$-clique of $G_c$ contains $h$ distinct $(h-1)$-cliques, $|\Lambda| = \bigO \left( h \mu_h(G_c) \right)$, where $\mu_h(G_c)$ is the number of $h$-cliques in $G_c$. Thus, the number of nodes in $\mathcal{H}$ is $\bigO \left( n_c + h \mu_h(G_c) \right)$, and the number of edges is $\bigO \left( n_c + \sum_{v \in V} deg_{G_c}(v, h) + (h - 1) h \mu_h(G_c) \right) = \bigO \left( n_c + h^2 \mu_h(G_c) \right)$.
% Also, computing $\rho_h^*$ (Line \ref{line:val}) requires $\bigO(n + |\Lambda|) = \bigO(n + h \mu_h(G))$ space \cite{FYCLX19}.
Since these constitute most of the memory consumed, the total space complexity of Algorithm \ref{alg:clique_densest} is $\bigO \left( n_c + h^2 \mu_h(G_c) \right)$.

Note that, when we adapt Algorithm \ref{alg:exact} for \textsf{$h$-Clique-MPDS}, in addition to the memory required for storing the uncertain graph,
the majority of the memory is consumed by Line \ref{line:all_densest}, which invokes Algorithm \ref{alg:clique_densest}. Denoting by $\mu_h^*$ the maximum number of $h$-cliques in the $(\lceil \Tilde{\rho} \rceil, h)$-core of any possible world of $\mathcal{G}$, the overall space complexity of our method is $\bigO \left( m + n + h^2 \mu_h^* \right)$.

\spara{Time complexity.} For Lines \ref{line:lb}-\ref{line:all_instance} in Algorithm \ref{alg:clique_densest}, the major step is enumerating all $h$-cliques in $G$, which takes $\bigO \left(hm \left( \frac{\mu_h(G)}{2} \right)^{h-2} \right)$ time, where $\mu_h(G)$ is the number of $h$-cliques in $G$ \cite{DBS18}. % Let $T_{val}$ denote the time taken to compute $\rho_h^*$ in Line \ref{line:val}.
%
% \textcolor{olive}{\bf [AK: Say more about $T_{val}$, how it depends on $G_c$, according to [54].]}
%
If $T$ denotes the number of iterations involved in computing $\rho_h^*$ using \cite{SDCS20}, the running time of Line \ref{line:val} consists of optimizing the convex program and computing the maximum flow in each iteration \cite{SDCS20}, and requires $\bigO \left( 2^T h \mu_h(G_c) + T \left( n_c h \mu_h(G_c) + n_c^3 \right) \right)$ time, where $n_c$ is as defined above.
% \textcolor{olive}{\bf [AK: Say what is $n_c$. It is already defined as maximum in \S 3.1]}
Lines \ref{line:begin_enum_all}-\ref{line:max_flow} can be done in $\bigO \left( \left( n_c h \mu_h(G_c) + n_c^3 \right) \right)$ time \cite{FYCLX19}.
%
% \textcolor{olive}{\bf [AK: Say why according to \cite{FYCLX19}.]}
%
Line \ref{line:scc} takes $\bigO \left( n_c + h^2 \mu_h(G_c) \right)$ time, as it involves finding the strongly connected components of $\mathcal{H}_{f^*}$, whose node and edge counts are stated above.
%
% \textcolor{olive}{\bf [AK: Say why.]}
%
In Line \ref{line:end_enum_all}, each densest subgraph is enumerated exactly once (as proved in Appendix \ref{sec:clique_proof}), and each subgraph enumeration takes time linear in the corresponding number of nodes.

Denoting respectively by $n_c^*$, $d^*$, $L^*$ and $T^*$, the maximum number (in the $(\lceil \Tilde{\rho} \rceil, h)$-core of any possible world) of nodes, densest subgraphs, nodes in a densest subgraph
% \textcolor{olive}{\bf [AK: total no of nodes where? is there any maximum here?]}
and iterations of \cite{SDCS20} to compute $\rho_h^*$, and by $\mu_h^*$ the maximum number of $h$-cliques in any possible world, the overall time complexity of our method is \small{$\bigO \left( \theta \left( h m \left( \frac{\mu_h^*}{2} \right)^{h-2} + 2^{T^*} h \mu_h^* + T^* \left( n_c^* h \mu_h^* + n_c^{*3} \right) + d^* L^* \right) \right)$}. \normalsize Practically, $n_c^* \ll n$ and $T^*$ is very small, as validated in our experiments (\S~\ref{sec:exp}). For instance, $T^* = $ \textcolor{olive}{XX}, $\frac{n_c^*}{n}$ = \textcolor{olive}{0.XX}, $d^*$ = \textcolor{olive}{XX}, $L^*$ = \textcolor{olive}{XX},  $\mu_h^*$ = \textcolor{olive}{XX}, for our largest \textcolor{olive}{ZZ} dataset, making our algorithm quite efficient with large-scale graphs.
% \textcolor{olive}{\bf [AK: Provide heuristic ways to improve the time complexity.]}

\spara{Accuracy guarantee.} We show (briefly in the following and in details in Appendix \ref{sec:clique_proof}) that Algorithm \ref{alg:clique_densest} correctly computes all $h$-clique-densest subgraphs in a deterministic graph. Therefore, our overall accuracy guarantees for finding the top-$k$
\textsf{$h$-Clique-MPDS} from an uncertain graph remain the same as in \S \ref{sec:top_k_mpds_algorithm}.
%
\begin{theor}
Given a deterministic graph $G$ and a positive integer $h$, Algorithm \ref{alg:clique_densest} enumerates each $h$-clique densest subgraph of $G$ exactly once.
\end{theor}
%
\begin{proof}
[Proof Sketch]
Lines \ref{line:lb}-\ref{line:core} of Algorithm \ref{alg:clique_densest} are justified by the fact that the densest subgraph is in the $(\lceil \rho_h^* \rceil, h)$-core, and hence in the $(\lceil \Tilde{\rho} \rceil, h)$-core \cite{FYCLX19}.
% \textcolor{olive}{\bf [AK: will this be $(\lceil \Tilde{\rho} \rceil, h)$-core? And does the correctness of $\rho_h^*$ follow from \cite{FYCLX19}?]}.
The correctness of Line \ref{line:val} follows from \cite{SDCS20}.
The main idea behind the remaining lines is that %the key to
all $h$-clique densest subgraphs of $G$ are hidden in the residual graph $\mathcal{H}_{f^*}$ of $\mathcal{H}$ under a maximum flow $f^*$.
Any $h$-clique densest subgraph of $G$ constitutes a minimum $s$-$t$ cut in $\mathcal{H}$, and thus there is no outgoing edge from that subgraph
in $\mathcal{H}_{f^*}$.
\end{proof}


==> old/3c-pattern_old.tex <==
\subsection{\textsf{Pattern-MPDS}: Approximate Algorithm}
\label{sec:pattern}

The overall algorithm and accuracy guarantees remain the same as in \S \ref{sec:top_k_mpds_algorithm}, except that in Line \ref{line:all_densest} of Algorithm \ref{alg:exact}, we need to find {\em all} pattern-densest subgraphs (w.r.t. a given pattern $\psi = (V_\psi, E_\psi)$) of the sampled possible world $G$. The method for doing so is inspired by \cite{FYCLX19, CQ20} and is shown in Algorithm \ref{alg:pattern_densest}. As earlier, {\em finding all pattern-densest subgraphs in a deterministic graph is a novel problem, and Algorithm \ref{alg:pattern_densest}
is one of our novel technical contributions.}

Algorithm \ref{alg:pattern_densest} is similar to Algorithm \ref{alg:clique_densest} (\S~\ref{sec:clique}); in fact, the $(k, h)$-core (Definition \ref{def:core}) can be easily extended to the $(k, \psi)$-core (which is computed in Line \ref{line:core_pat}), and $\rho_\psi^*$ can be computed in Line \ref{line:val_pat} by extending \cite{SDCS20}. Nevertheless, there are two main differences. First, in Line \ref{line:all_instance}, $\Lambda$ refers to the set of all $\psi$-instances in $G$, which can be enumerated using the method in \cite{QZC17}. 
Second, the flow network $\mathcal{H}$ (constructed as in \cite{FYCLX19}, with the pseudocode included in Appendix \ref{sec:pattern_proof}) contains one node for each group of $\psi$-instances with a common node set, instead of one for each instance, in order to reduce the memory footprint and running time. This forms the main difference between our method and the one in \cite{CQ20}, resulting in some non-trivial additions which constitute one of our novel contributions.
% Second, in Algorithm \ref{alg:flow_pat}, distinct nodes are not created for each $\psi$-instance. Rather, the instances are grouped based on the node set \textcolor{olive}{\bf [AK: what node set?]}, and one node $\lambda'$ is constructed for each such group $g'$ \textcolor{olive}{\bf [AK: not clear]}. For each $v' \in \lambda'$, the edge $(v', \lambda')$ has capacity $|g'|$ and the edge $(\lambda', v')$ has capacity $|g'| \left( \left| V_\psi \right| - 1 \right)$ \textcolor{olive}{\bf [AK: not clear. Moreover, what is the usefulness of such differences w.r.t. Alg-2?] [AK: Why Alg-3, 6 has two citations, are these not original? If inspired by them, no need to mention the citations in algorithm block]}.
% Second, Algorithm \ref{alg:flow} cannot be trivially extended for general patterns since it relies on $(h-1)$-cliques. Nevertheless, we can adapt the flow network construction in \cite{T15} by replacing the steps of computing all clique instances with pattern instances. The resulting algorithm, which creates one node in the flow network for each pattern instance, can be further optimized by the following key observation: For a general pattern $\psi$, different instances in $\Lambda$ may share the same set of nodes in $V$. Thus, we can create groups of pattern instances in $\Lambda$, with the instances in one group sharing the same set of nodes in $V$, and create one node in the flow network for each such group. This makes the flow network smaller, resulting in better memory usage and running time. This optimized method is shown in Algorithm \ref{alg:flow_pat}.

% \textcolor{olive}{\bf [AK: the following algorithms and descriptions are repetitive. If they are very similar to \S~\ref{sec:clique}, perhaps we just mention the difference in this section, without being so much detailed.]}

\begin{algorithm}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\scriptsize
	\caption{\small Find all pattern-densest subgraphs} \label{alg:pattern_densest}
	\begin{algorithmic}[1]
		\REQUIRE Deterministic graph $G = (V,E)$, pattern $\psi = (V_\psi, E_\psi)$
		\ENSURE All pattern-densest subgraphs w.r.t. $\psi$ in $G$
		\STATE $\Tilde{\rho} \gets $ Density returned by the peeling method \cite{FYCLX19} \label{line:lb_pat}
		\STATE $G \gets (\lceil \Tilde{\rho} \rceil, \psi)$-core of $G$ \cite{FYCLX19} \label{line:core_pat}
		\STATE $\Lambda \gets $ All $\psi$-instances in $G$ \label{line:all_instance_pat}
		\STATE $\rho_\psi^* \gets \max_{S \subseteq V} \rho_\psi(S)$ \cite{SDCS20} \label{line:val_pat}
		\STATE $\mathcal{H} \gets $ Alg. \ref{alg:flow_pat} ($G$, $\psi$, $\Lambda$, $\rho_h^*$) \cite{FYCLX19} \label{line:begin_enum_all_pat}
		\STATE $f^* \gets $ Maximum flow in $\mathcal{H}$ \label{line:max_flow_pat}
		\STATE $\mathcal{C} \gets $ SCCs of the residual graph $\mathcal{H}_{f^*}$, excluding those of $s$ and $t$ \label{line:scc_pat}
		\RETURN Alg. \ref{alg:enum} ($\emptyset$, $\mathcal{C}$, $V$) \label{line:end_enum_all_pat}
	\end{algorithmic}
\end{algorithm}

\spara{Accuracy guarantee.} By a similar analysis as in Appendix \ref{sec:clique_proof}, it can be shown that Algorithm \ref{alg:pattern_densest} correctly computes all pattern-densest subgraphs w.r.t. $\psi$ in a deterministic graph. The main difference is in the derivation of the capacity of a minimum cut in $\mathcal{H}$, which is quite different from the one in \S~\ref{sec:clique} as mentioned above; this derivation is shown in Appendix \ref{sec:pattern_proof}. Finally, since Algorithm \ref{alg:pattern_densest} correctly computes all pattern-densest subgraphs w.r.t. $\psi$ in a deterministic graph, our overall accuracy guarantees for finding the top-$k$ 
\textsf{pattern-MPDS} from an uncertain graph remain the same as in \S \ref{sec:top_k_mpds_algorithm}.

\spara{Space complexity.} Let $G_c$ be the $(\lceil \Tilde{\rho} \rceil, \psi)$-core in Lines \ref{line:lb}-\ref{line:core} of Algorithm \ref{alg:pattern_densest}, with $n_c$ and $m_c$ the corresponding node and edge counts, respectively. Clearly $|\Lambda| = \bigO \left( \mu_\psi(G_c) \right)$, where $\mu_\psi(G_c)$ is the number of $\psi$-instances in $G_c$. Thus, the number of nodes in $\mathcal{H}$ is $\bigO \left( n_c + \mu_\psi(G_c) \right)$, and the number of edges is $\bigO \left( n_c + \left| V_\psi \right| \mu_\psi(G_c) \right)$. Also, computing $\rho_\psi^*$ (Line \ref{line:val_pat}) requires $\bigO(n_c + |\Lambda|) = \bigO(n_c + \mu_\psi(G_c))$ space \cite{FYCLX19}. Since these constitute most of the memory consumed, the total space complexity of Algorithm \ref{alg:pattern_densest} is $\bigO \left( n_c + \left| V_\psi \right| \mu_\psi(G_c) \right)$.

Note that, when we adapt Algorithm \ref{alg:exact} for \textsf{Pattern-MPDS}, in addition to the memory required for storing the uncertain graph, the majority of the memory is consumed by Line \ref{line:all_densest}, which invokes Algorithm \ref{alg:pattern_densest}. Denoting by $\mu_\psi^*$ the maximum number of $\psi$-instances in the $(\lceil \Tilde{\rho} \rceil, h)$-core of any possible world of $\mathcal{G}$, the overall space complexity of our method is $\bigO \left( m + n + \left| V_\psi \right| \mu_\psi^* \right)$.

\spara{Time complexity.} Assume that the enumeration of all $\psi$-instances in a possible world takes $\bigO(t_{\psi})$ time. By a similar analysis as in \S~\ref{sec:clique}, denoting respectively by $n_c^*$, $d^*$, $L^*$, $\mu_\psi^*$ and $T^*$, the maximum number (in the $(\lceil \Tilde{\rho} \rceil, \psi)$-core of any possible world) of nodes, densest subgraphs, nodes in a densest subgraph, 
% \textcolor{olive}{\bf [AK: total no of nodes where? is there any maximum here?]}
$\psi$-instances, and iterations of \cite{SDCS20} to compute $\rho_\psi^*$, the overall time complexity of our method is $\bigO \left( \theta \left( t_{\psi} + 2^{T^*} \left| V_\psi \right| \mu_\psi^* + T^* \left( n_c^* \mu_\psi^* + n_c^{*3} \right) + d^* L^* \right) \right)$.
% \textcolor{olive}{\bf [AK: Add time complexity assuming some pattern enumeration complexity. Provide heuristic ways to improve the time complexity.]}

\spara{Remark.} For larger graphs and bigger patterns $\psi$, we find that the enumeration of all $\psi$-instances (which is necessary to compute the densest subgraphs in a possible world) can be expensive. In such cases, we resort to a heuristic method in which we enumerate reasonably dense subgraphs (instead of the densest ones) using \cite{FYCLX19}.
% \textcolor{olive}{\bf [AK: \cite{FYCLX19} can enumerate one reasonably dense subgraph in Line 4. What happens in Lines 5-8?]}
Specifically, we use a different algorithm (than Algorithm~\ref{alg:pattern_densest}) which runs core decomposition w.r.t. $\psi$. If $k_{max}$ denotes the maximum core number, then the $(k_{max}, \psi)$-core is a reasonably dense subgraph. In particular, the $(k_{max}, \psi)$-core's density is at least $\frac{1}{\left| V_{\psi} \right|}$-times the maximum density of any subgraph \cite{FYCLX19}. Based on this, we return the $(k_{max}, \psi)$-core and all intermediate subgraphs (obtained during core decomposition) having greater densities.
Experimental results (\S~\ref{sec:large_graph_results}) show that this heuristic method yields good-quality solutions with higher efficiency.


==> old/4-approx.tex <==
\section{Approximate Solution for \\ Nucleus Densest Subgraphs}
\label{sec:nucleus}

Our approximate method to enumerate all nucleus densest subgraphs, or {\sf NDS}
(for all three notions of density:
edge density, h-clique density, and pattern density)
is shown in Algorithm \ref{alg:exact_nucleus}. Briefly, it first runs $\theta$ independent rounds of the following: Sample a possible world $G \sqsubseteq G$ and find the union $S$ of all densest subgraphs of $G$, which is inserted into the set of candidate node sets $CV$. After $\theta$ rounds, it uses a frequent itemset mining algorithm (e.g., \textsf{FP-Growth} \cite{HPY00}) to compute the node sets that are contained in at least $\sigma\theta$ out of $\theta$ node sets in $CV$. {\em The novelty of our solution is that we convert the {\sf NDS} problem into the widely-studied frequent itemsets mining problem}.
Here, $\sigma \in [0, 1]$ is as defined in Problem \ref{prob:cont_min} and is provided by the user as an input; its value is decided based on the minimum desired probability of the returned node sets being contained in a densest subgraph. Too small values lead to longer running times, while too large values increase the chances of getting an empty node set.

% \textcolor{olive}{\bf [AK: What is $\sigma$, e.g., an input, how the user decides it? Mention in one sentence its impact on accuracy vs. efficiency.]}

\begin{algorithm}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\scriptsize
	\caption{\small Estimate all \textsf{NDS} in an uncertain graph} \label{alg:exact_nucleus}
	\begin{algorithmic}[1]
		\REQUIRE Uncertain graph $\mathcal{G} = (V,E,p)$, positive threshold $\sigma$, and no. of samples $\theta$
		\ENSURE (Approximate) \textsf{NDS}
		\STATE $CV \gets \emptyset$
		\FOR{$i = 1$ \TO $\theta$}
		\STATE Sample a possible world $G \sqsubseteq \mathcal{G}$
		\STATE $S \gets$ Maximal densest subgraph in $G$ \label{line:all_densest_nucleus}
		\STATE $CV \gets CV \cup \{S\}$
		\ENDFOR
		\RETURN \textsf{FP-Growth}($CV$, $\sigma\theta$) \cite{HPY00}
	\end{algorithmic}
\end{algorithm}

The rationale behind computing the union of all densest subgraphs is as follows. By a trivial generalization of \cite{BBCGS15} to all notions of density, for a deterministic graph $G$, the union of all densest subgraphs of $G$ is a densest subgraph of $G$; this is called the maximal densest subgraph of $G$. Thus, it is easy to see that a node set $U \subseteq V$ is contained in a densest subgraph of $G$ if and only if it is contained in the maximal densest subgraph of $G$.

The maximal densest subgraph in a deterministic graph (Line \ref{line:all_densest_nucleus}) can be computed using parts of the methods in \S~\ref{sec:mpds_algo}. For edge density, we can terminate after computing the SCCs of the residual graph under a maximum flow \cite{CQ20}. For clique and pattern densities, we can terminate after computing the value of the maximum density of a subgraph, since in that process we also get the maximal densest subgraph \cite{SDCS20}.

% The usage of a frequent itemset mining algorithm is justified by the fact that all node sets satisfy the apriori property.

\spara{Space complexity.} The majority of the memory is consumed by the flow network in each iteration of Algorithm \ref{alg:exact_nucleus}, and hence the overall space complexity is the same as in \S~\ref{sec:mpds_algo}.

\spara{Time complexity.} The time complexity is similar to the ones in \S~\ref{sec:mpds_algo},
%minus the time required for computing all densest subgraphs in the sampled possible worlds ($\bigO(\theta d^*L^*)$ in \S~\ref{sec:mpds_algo}),
plus that taken to compute the frequent node sets using \textsf{FP-Growth}, which is reasonable in our experiments (\S~\ref{sec:parameter}).
% which is $\bigO \left( c^2 d \right)$, where $c$ is the header count and $d$ is the depth of the FP-tree \cite{singh2013performance}. Both $c$ and $d$ are upper-bounded by the number of distinct items, which is at most $n_c^*$ (defined in \S~\ref{sec:mpds_algo}).
% \textcolor{red}{[AK: Some empirical evidences should be given on the efficiency of \textsf{FP-Growth} on our datasets. Otherwise, is there a formal time-complexity of it?]}
Note that, for \textsf{Pattern-NDS} on our larger graphs, we use the heuristic method of \S~\ref{sec:pattern} in Line \ref{line:all_densest_nucleus} of Algorithm \ref{alg:exact_nucleus}.


\spara{Accuracy guarantee.} We show that a node set $U$ with a higher probability $\gamma(U)$ of being contained in a densest subgraph, is also highly likely to be returned by our method.

\begin{theor}
\label{th:nucleus}
Consider a node set $U \subseteq V$
having probability $\gamma(U)$ of being contained in a densest subgraph.
Let $\widehat{\gamma}(U)$ denote the fraction of candidate node sets $U' \in CV$ such that $U \subseteq U'$. If $\gamma(U) > \sigma$ (resp. $\gamma(U) < \sigma$), then $\widehat{\gamma}(U) > \sigma$ (resp. $\widehat{\gamma}(U) < \sigma$) with probability at least: $1 - \exp \left( -2 \theta \left| \gamma(U) - \sigma \right| ^2 \right)$.
\end{theor}
%
\begin{proof}
Let $X_i(U)$ be a binary random variable denoting whether $U$ is contained in the maximal densest subgraph in the $i^{th}$ possible world; thus $\widehat{\gamma}(U)$ = $\frac{1}{\theta} \sum_{i=1}^\theta X_i(U)$. Clearly, $\mathbbm{E}[X_i(U)]$ = $\Pr \left( X_i[U] = 1 \right)$ = $\gamma(U)$; hence $\mathbbm{E}[\widehat{\gamma}(U)] = \gamma(U)$.


Now, suppose $\gamma(U) > \sigma$. From Hoeffding's inequality,
\begin{small}
\begin{align*}
    \Pr \left( \widehat{\gamma}(U) > \sigma \right) &= 1 - \Pr \left( \widehat{\gamma}(U) - \gamma(U) \leq -\left| \gamma(U) - \sigma \right| \right) \\
    &\geq 1 - \exp \left( -2 \theta \left| \gamma(U) - \sigma \right| ^2 \right)
\end{align*}
\end{small}
A similar proof applies for the case when $\gamma(U) < \sigma$.
\end{proof}

% \textcolor{olive}{\bf [AK: Discuss accuracy-efficiency trade-off w.r.t. $\theta$, $\sigma$.]}

We now discuss the impact of $\theta$ and $\sigma$ on the accuracy and the efficiency of Algorithm \ref{alg:exact_nucleus}. Increasing $\theta$ implies higher chances of more accurate results (Theorem \ref{th:nucleus}), at the cost of a longer running time. If $\sigma$ is too small, then the running time increases because the number of frequent node sets increases. In contrast, if $\sigma$ is too large, then the chances of an empty node set being returned increase, as the returned node set needs to be contained in a larger number of candidate subgraphs. 

==> old/5-related.tex <==
\section{Related Work}
\label{sec:related}
To the best of our knowledge, the problem of finding the top-$k$ most probable densest subgraphs
in an uncertain graph, that we study in this work, is novel. In the following, we provide an overview
of relevant work in neighboring areas.

\spara{Maximum expected edge densest subgraph.}
The expected edge density of a node set $U$ in the uncertain graph $\mathcal{G}$ is $\sum_{G \sqsubseteq \mathcal{G}}Pr(G)\cdot \rho(G[U])$,
where $G$ is a possible world of $\mathcal{G}$, the subgraph induced by the node set $U$ in $G$ is denoted by $G[U]$,
and $\rho(G[U])$ is the edge density of $G[U]$ in $G$. Zou \cite{Zou13} designed a polynomial-time algorithm to find the
maximum expected edge densest subgraph in an uncertain graph using maximum flow techniques. As shown in Example~\ref{exam:expected}
and in our experiments (\S \ref{sec:comp_others}), the maximum expected edge densest subgraph is different from {\sf MPDS}:
a subgraph of the uncertain graph having the maximum expected edge density may induce densest subgraphs
{\em only in a few} possible worlds of that uncertain graph. Such a subgraph can be large with many
low-probability edges, or having nodes that are loosely connected.

\spara{Core and truss decompositions in an uncertain graph.}
As cohesive and dense substructures finding, core and truss decompositions are popular. The $k$-core of a graph is a maximal subgraph
in which every node is connected to at least $k$ other nodes within that subgraph. Analogously, the $k$-truss is defined as a 
maximal subgraph in which each edge participates in at least $(k-2)$ triangles within that subgraph. These notions have been 
extended to uncertain graphs in \cite{BonchiGKV14,EsfahaniW0T019,SMPV17,Dai21,HuangLL16,Sun0XB21,ZouZ17}. The inner cores and trusses 
have been used in applications such as task-driven team formation due to their higher densities \cite{HuangLL16,BonchiGKV14}. However,
the innermost cores and trusses are different from the {\sf MPDS} as we depict in our empirical results (\S \ref{sec:comp_others} and \S \ref{sec:case_club}). 
Unlike the {\sf MPDS}, they do not find the node set that is the most likely to induce a densest subgraph in the uncertain graph.

\spara{Top-k maximal cliques in an uncertain graph.} A clique is a set of nodes with each pair of nodes connected by an edge.
Enumeration of maximal cliques in uncertain graphs have been studied in \cite{MukherjeeXT17,ZouLGZ10,LiDWMQY19}. Clearly,
cliques and densest subgraphs are two different concepts. 

\spara{Node clustering in an uncertain graph.} $k$-mean and $k$-median approaches are extended to cluster nodes in an uncertain
graph \cite{LJAS12,HanGXTHCH19,CeccarelloFPPV17}: partition the nodes into $k$ clusters such that some notion of path-based 
connection probability (e.g., reliability) between each node and its cluster's center 
(or, across each pair of nodes within every cluster) is maximized.
Notice that clustering methods optimize the path-based connection probability between nodes inside a cluster, and do not optimize
the density of a subgraph. 

\spara{Highly reliable subgraphs in an uncertain graph.} Jin et al. \cite{JinLA11} have developed a mining-based approach to 
discover highly reliable subgraphs in an uncertain graph. A highly reliable subgraph denotes a node set that has
a high probability of remaining connected via some paths in possible worlds of the uncertain graph. This method deals with 
path-based connectivity between nodes, and thus not suitable to identify densest subgraphs, such as {\sf MPDS} as in our work.




